ProCLIP: Progressive Vision-Language Alignment via LLM-based Embedder

The original CLIP text encoder is limited by a maximum input length of 77 tokens, which hampers its ability to effectively process long texts and perform fine-grained semantic understanding. In addition, the CLIP text encoder lacks support for multilingual inputs. All these limitations significantly restrict its applicability across a broader range of tasks. Recent studies have attempted to replace the CLIP text encoder with an LLM-based embedder to enhance its ability in processing long texts, multilingual understanding, and fine-grained semantic comprehension. However, because the representation spaces of LLMs and the vision-language space of CLIP are pretrained independently without alignment priors, direct alignment using contrastive learning can disrupt the intrinsic vision-language alignment in the CLIP image encoder, leading to an underutilization of the knowledge acquired during pre-training. To address this challenge, we propose ProCLIP, a curriculum learning-based progressive vision-language alignment framework to effectively align the CLIP image encoder with an LLM-based embedder. Specifically, ProCLIP first distills knowledge from CLIP's text encoder into the LLM-based embedder to leverage CLIP's rich pretrained knowledge while establishing initial alignment between the LLM embedder and CLIP image encoder. Subsequently, ProCLIP further aligns the CLIP image encoder with the LLM-based embedder through image-text contrastive tuning, employing self-distillation regularization to avoid overfitting. To achieve a more effective alignment, instance semantic alignment loss and embedding structure alignment loss are employed during representation inheritance and contrastive tuning. The Code is available at https://github.com/VisionXLab/ProCLIP.

==> Table/MMVP.tex <==
\begin{wraptable}[]{r}{0.6\textwidth}

\centering
\captionsetup{font=small}
\caption{MMVP performance. The best results are marked in \textbf{bold}.}
\vspace{-2mm}
\label{tab:roubutness}
\resizebox{0.6\textwidth}{!}{
\begin{tabular}{lccccccccccc}
\toprule
\multirow{2}{*}{\textbf{Method}}  &\multirow{2}{*}{\textbf{Data}} & \multicolumn{10}{c}{\textbf{MMVP}} \\

& &  \faCompass &  \textbf{IN-A} &   \textbf{IN-O}&   \textbf{IN-R}&\textbf{IN-S} \\
\midrule
\multicolumn{4}{l}{\textit{Model Architecture: CLIP ViT-L/14}} & &   \\
\textcolor{gray}{CLIP} & 
\textcolor{gray}{400M} & 
\textcolor{gray}{69.8} & 
\textcolor{gray}{70.8} & 
\textcolor{gray}{32.2} & 
\textcolor{gray}{87.8} & 
\textcolor{gray}{59.6} \\


\bottomrule
\end{tabular}
}
\vspace{-3mm}
\end{wraptable}




==> Table/ablation.tex <==
\begin{table*}[t!]
\centering
\caption{Ablation}
\label{tab:ablation}
\resizebox{0.6\linewidth}{!}{
\begin{tabular}{cccccc} %
\toprule


index & method & ImageNet & I2T Avg. & T2I Avg. \\
\midrule
0 & LLM2CLIP & 52.8 & 82.0 & 79.1 \\
\hline
1 & +$\mathcal{L}_{\text{ins}}$& 58.9 & 69.3 &59.4\\
2 & +$\mathcal{L}_{\text{struct}}$ & 59.5 &70.3 &  61.2  \\
\hline
3 & +$\mathcal{L}_{\text{info}}$ & 59.2 &82.9 & 80.2   \\
4  & +$\mathcal{L}_{\text{reg}}$ & 62.5 & 83.0 & 80.5 \\

\bottomrule
\end{tabular}
}

\vspace{-5mm}
\end{table*}

==> Table/ablation_new.tex <==
\begin{table}[t!]
\centering 
\label{tab:ablation}
\begin{tabular}{cc|cccc|ccc}
\toprule
\textbf{\#} &
\textbf{Method} & 
\textbf{$\mathcal{L}_{\text{ins}}$} & \textbf{$\mathcal{L}_{\text{struct}}$} & \textbf{$\mathcal{L}_{\text{info}}$} & \textbf{$\mathcal{L}_{\text{reg}}$}  & \textbf{IN-1k} & \textbf{I2T Avg} & \textbf{T2I Avg} \\
\midrule
 0  & \textcolor{gray}{CLIP} & & & & &   \textcolor{gray}{74.5} & \textcolor{gray}{66.9} &\textcolor{gray}{55.5} \\
 1 & 
\textcolor{gray}{LLM2CLIP} & & & & &  \textcolor{gray}{52.8} & \textcolor{gray}{82.0} & \textcolor{gray}{79.1}   \\
\midrule
2 & \multirow{4}{*}{ProCLIP} & \ding{51} & & & & 58.9 & 69.3 & 79.4 \\
3 &                          & \ding{51} & \ding{51} & & & 59.5 & 70.3 & 61.2 \\
4 &                          & \ding{51} & \ding{51} & \ding{51} & & 59.2 & 82.9 & 80.2 \\
5 &                          & \ding{51} & \ding{51} & \ding{51} & \ding{51} & 62.5 & 83.0 & 80.5 \\
\bottomrule
\end{tabular}
\caption{Ablation of different components.}
\vspace{-3mm}

\end{table}


==> Table/clip_eva_siglip.tex <==
\begin{table}[t!]
    \centering
    \caption{Ablation study on different base model architectures. All methods use 3M training samples.}
    \setlength{\tabcolsep}{3pt}
    \resizebox{1.0\linewidth}{!}{
    \begin{tabular}{llccc}
        \toprule
        \textbf{Base Model} & \textbf{Method} & \textbf{IN-1k} & \textbf{I2T Avg.} & \textbf{T2I Avg.} \\
        \midrule
        \multirow{2}{*}{CLIP ViT-L}        
        & LLM2CLIP & 52.8 & 82.0 & 79.1 \\
        & \cellcolor[rgb]{0.925,0.957,1}ProCLIP  & \cellcolor[rgb]{0.925,0.957,1}\textbf{62.5} & \cellcolor[rgb]{0.925,0.957,1}\textbf{83.0} & \cellcolor[rgb]{0.925,0.957,1}\textbf{80.5} \\
        \midrule
        \multirow{2}{*}{EVA02-CLIP ViT-L}
        & LLM2CLIP & 56.4 & 83.6 & 80.9 \\
        & \cellcolor[rgb]{0.925,0.957,1}ProCLIP  & \cellcolor[rgb]{0.925,0.957,1}\textbf{66.8} & \cellcolor[rgb]{0.925,0.957,1}\textbf{84.2} & \cellcolor[rgb]{0.925,0.957,1}\textbf{82.2} \\
        \midrule
        \multirow{2}{*}{SigLIP2 SO/14@224}
        & LLM2CLIP & 63.8 & 84.6 & 81.9 \\
        & \cellcolor[rgb]{0.925,0.957,1}ProCLIP  & \cellcolor[rgb]{0.925,0.957,1}\textbf{67.7} & \cellcolor[rgb]{0.925,0.957,1}\textbf{86.3} & \cellcolor[rgb]{0.925,0.957,1}\textbf{83.9} \\
        \bottomrule
    \end{tabular}
    }
\vspace{-3mm}
\label{tab:ablation_arch}
\end{table}

==> Table/different_llm_embedder.tex <==
\begin{table*}[t!]
\centering
\caption{Ablati}
\label{tab:llm_embedder}
\resizebox{0.6\linewidth}{!}{
\begin{tabular}{cccc} %
\toprule

LLM embedder & ImageNet & I2T Avg. & T2I Avg. \\
\midrule

Qwen3-embedding 0.6B & 41.4 & 54.7 & 51.7  \\


Qwen3-embedding 4B &49.9  &  80.2 & 77.5\\

Qwen3-embedding 8B & 51.8  & 82.2 & 79.0\\

 GME-8B & 55.4  & 83.8&  79.7 \\

 Nv-embedddingv2 & 56.2 & 82.6 & 79.3 \\
 LLama-cc & 57.0 & 83.2 & 80.1\\

\bottomrule
\end{tabular}
}

\vspace{-5mm}
\end{table*}

==> Table/liner_probe_new.tex <==
\begin{table*}[t!]
\centering
\caption{Linear Probe performance on 11 datasets. The best results are marked in bold, and the second-best results are underlined. }
\vspace{-3mm}
\label{tab:linear}
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{lcccccccccccc|c}
\toprule
\textbf{Method}  &\textbf{Data} &  \rotatebox{90} {\textbf{Food101}} & \rotatebox{90} {\textbf{CIFAR10}} &  \rotatebox{90} {\textbf{CIFAR100}}& \rotatebox{90} {\textbf{SUN397}} & \rotatebox{90} {\textbf{Cars}} & \rotatebox{90} {\textbf{Aircraft}}& \rotatebox{90} {\textbf{DTD}} & \rotatebox{90} {\textbf{Pets}}  & \rotatebox{90} {\textbf{Caltech101}} &  \rotatebox{90} {\textbf{Flowers}}  & \rotatebox{90} {\textbf{ImageNet}} & \textbf{Avg.} \\
\hline
\multicolumn{14}{c}{\textbf{\textit{Model Architecture: CLIP ViT-B/32}}} \\
\hline
\textcolor{gray}{CLIP} & 
\textcolor{gray}{400M} & 
\textcolor{gray}{88.6} & 
\textcolor{gray}{95.1} & 
\textcolor{gray}{80.1} & 
\textcolor{gray}{73.4} & 
\textcolor{gray}{80.8} & 
\textcolor{gray}{44.9} & 
\textcolor{gray}{76.3} & 
\textcolor{gray}{89.3} & 
\textcolor{gray}{92.7} & 
\textcolor{gray}{94.7} & 
\textcolor{gray}{-} & 
\textcolor{gray}{-}\\
\
LLM2CLIP & 3M & 87.9 & 95.7 & 83.1 & 74.1 & 78.0 & 44.9 & 77.7 & 90.4 & 92.4 & 94.6 & - & - \\
ProVLA & 3M & 88.4 & 95.9 & 83.1 & 74.3 & 79.5 & 44.1 & 78.2 & 90.3 & 92.6 & 95.0 & - & -\\

\hline
\multicolumn{14}{c}{\textbf{\textit{Model Architecture: CLIP ViT-B/16}}} \\
\hline
\textcolor{gray}{CLIP} & 
\textcolor{gray}{400M} & 
\textcolor{gray}{92.7} & 
\textcolor{gray}{96.0} & 
\textcolor{gray}{82.5} & 
\textcolor{gray}{75.7} & 
\textcolor{gray}{85.9} & 
\textcolor{gray}{52.8} & 
\textcolor{gray}{78.9} & 
\textcolor{gray}{93.1} & 
\textcolor{gray}{93.9} & 
\textcolor{gray}{96.4} & 
\textcolor{gray}{-} & 
\textcolor{gray}{-}\\


LLM2CLIP & 3M & 91.6 & 97.0 & 84.5 & 76.0 & 82.1 & 50.1 & 80.3 & 92.3 & 93.6 & 95.7 & &  \\
ProVLA & 3M & 92.8 & 96.8 & 84.6 & 76.4 & 85.6 & 52.0 & 80.6 & 93.3 & 94.2 & 97.0 &  & \\
\hline
\multicolumn{14}{c}{\textbf{\textit{Model Architecture: CLIP ViT-L/14}}} \\
\hline
\textcolor{gray}{CLIP} & 
\textcolor{gray}{400M} & 
\textcolor{gray}{95.3} & 
\textcolor{gray}{89.1} & 
\textcolor{gray}{87.2} & 
\textcolor{gray}{79.4} & 
\textcolor{gray}{90.7} & 
\textcolor{gray}{63.0} & 
\textcolor{gray}{81.8} & 
\textcolor{gray}{95.3} & 
\textcolor{gray}{96.9} & 
\textcolor{gray}{98.8} & 
\textcolor{gray}{-} & 
\textcolor{gray}{-} \\

LLM2CLIP & 3M & 94.5  & 98.6 & 89.2 & 79.6 & 86.7 & 57.7 & 83.4 & 94.1 & 96.4 & 97.1 & -  & - \\
ProVLA & 3M & 95.3 & 98.5 & 88.8 & 80.3 & 90.3 & 61.0 & 83.6 & 95.2 & 96.9 & 98.7 & - & - \\


\hline
\multicolumn{14}{c}{\textbf{\textit{Model Architecture: EVA02-CLIP ViT-L/14}}} \\
\hline
\textcolor{gray}{EVA02-CLIP} & \textcolor{gray}{2B} & 
\textcolor{gray}{95.6} & 
\textcolor{gray}{99.5} & 
\textcolor{gray}{94.2} & 
\textcolor{gray}{80.4} & 
\textcolor{gray}{94.2} & 
\textcolor{gray}{69.5} & 
\textcolor{gray}{85.0} & 
\textcolor{gray}{94.8} & 
\textcolor{gray}{97.6} & 
\textcolor{gray}{99.4} \\


LLM2CLIP & 3M & 94.1 & 99.5 & 93.3 & 79.4 & 85.0 & 54.3 & 93.2 & 84.0 & 97.3 & 96.9  \\
ProVLA  & 3M & 95.3 & 99.5 & 94.0 & 81.0 & 93.9 & 65.7 & 85.9 & 95.4 & 97.8 & 99.3 \\
\bottomrule
\end{tabular}
}
\vspace{-3mm}
\end{table*}

==> Table/long_clip_compare.tex <==
\begin{table*}[t!]
\centering
\caption{Compared with Long-CLIP and VLM2Vec on multiple cross-modal retrieval datasets.}
\resizebox{1.0\textwidth}{!}{
\begin{tabular}{lcccccccccccccc}%
\toprule
\multirow{2}{*}{\textbf{Method}} &
\multicolumn{2}{c}{\textbf{Flickr30k}} & \multicolumn{2}{c}{\textbf{COCO}} &
\multicolumn{2}{c}{\textbf{ShareGPT4V}} & \multicolumn{2}{c}{\textbf{Urban-1k}} &
\multicolumn{2}{c}{\textbf{DOCCI}} & \multicolumn{2}{c}{\textbf{DCI}} & 
\multicolumn{2}{c}{\textbf{Avg.}} \\
 & I2T & T2I & I2T & T2I & I2T & T2I & I2T & T2I & I2T & T2I & I2T & T2I & I2T & T2I \\
\midrule
\textcolor{gray}{CLIP}  &  
\textcolor{gray}{86.6} & \textcolor{gray}{64.6} & %
\textcolor{gray}{57.2} & \textcolor{gray}{36.4} & %
\textcolor{gray}{78.0} & \textcolor{gray}{68.7} & %
\textcolor{gray}{68.4} & \textcolor{gray}{56.0} & %
\textcolor{gray}{65.8} & \textcolor{gray}{63.1} & %
\textcolor{gray}{45.4} & \textcolor{gray}{43.9} & %
\textcolor{gray}{66.9} & \textcolor{gray}{55.5} \\ %

Long-CLIP & 89.7 & 75.7 & 62.5 & 46.4 & 93.3 & 92.1 & 82.4 & 86.2 &  66.4 & 78.6 & 57.2 & 64.0 & 75.2 & 73.8     \\
VLM2Vec (LLaVA1.6) & 88.3 & 76.0 & 66.6 & 46.8 & 89.9 & 89.4 & 80.6 & 82.3 & 66.4 & 77.2 & 69.7  &72.0 & 76.9 & 74.0  \\ 
\rowcolor[rgb]{0.925,0.957,1}
ProCLIP(ViT-L-1M)  & \textbf{92.1} & \textbf{81.0} & \textbf{65.8} & \textbf{51.1} & 
\textbf{94.7} & \textbf{93.6}  & \textbf{85.0} & \textbf{91.0} & \textbf{84.8} & \textbf{86.6} & \textbf{68.7} & \textbf{74.7} & \textbf{81.9} & \textbf{79.7} \\
\bottomrule
\end{tabular}
}
\vspace{-3mm}
\label{tab:long_CLIP_com_pare}
\end{table*}

==> Table/more_comparision.tex <==
\begin{table*}[t!]
\centering
\caption{More Comparison with Previous Works.}
\vspace{-3mm}
\label{tab:more_comparison}
\resizebox{\linewidth}{!}{
\begin{tabular}{lllcccccc} %
\toprule


\multirow{2}{*}{\textbf{Method}} &
\multirow{2}{*}{\textbf{ViT init}} &
\multirow{2}{*}{\textbf{LLM embedder}} & 
\multirow{2}{*}{\textbf{Data}} &
\multirow{2}{*}{\textbf{ImageNet}} &
\multicolumn{2}{c}{\textbf{COCO}} &
\multicolumn{2}{c}{\textbf{Flickr30k}} \\
& & & &  & 
\textbf{I2T} & \textbf{T2I} &
\textbf{I2T} & \textbf{T2I} \\
\midrule
 FLAME & random & Mistral-Nemo &  3M & 36.0 & 43.3 & 28.6 & 67.3 & 53.6\\

 ShareLock & DINOv2 B/14  &   Llama3 &3M& 52.1 & - & -& -\\ 

LIFT & random & NV-Embedv2 & 512M & 43.6 & 34.6 & 36.0 & 69.1 & 72.9  \\
LIFT & random & NV-Embedv2 & 1.28B & \textbf{58.3} & 29.1 & 28.1 & 58.8 & 63.7\\


LLM2CLIP &CLIP B/16 & Llama3-CC &  3M & 45.8 & 60.5 & 44.8 & 88.0 & 75.3 \\


\rowcolor[rgb]{0.925,0.957,1}ProCLIP &CLIP B/16 & Llama3-CC &  3M & 54.8 & \textbf{61.7} & \textbf{46.8} & \textbf{89.4} & \textbf{77.6} \\

\midrule

SAIL & DINOv2 L/14 & NV-Embedv2 & 3M & 54.0 & 45.4 & 32.9 & - & - \\ 

LiT &CLIP L/14 & Llama3-cc &  3M & 60.1 & 59.4 & 44.6 & 88.0 & 74.7   \\

LLM2CLIP &CLIP L/14 & Llama3-cc &  3M & 52.8 & 65.5 & 49.7 & 92.4 & 80.1   \\
\rowcolor[rgb]{0.925,0.957,1}ProCLIP &CLIP L/14& NV-Embedv2 &  3M & 61.4  & 64.8 & 51.7 & 91.9 & \textbf{81.4} \\
\rowcolor[rgb]{0.925,0.957,1}ProCLIP &CLIP L/14& Llama3-CC &  3M & \textbf{62.5} &  \textbf{66.4} & \textbf{51.9} & \textbf{92.8} & 81.1  \\




\bottomrule
\end{tabular}
        }

\vspace{-5mm}
\end{table*}

==> Table/multilingual.tex <==

\begin{table*}[t!]
\centering
\caption{Crossmadal3600 retrieval.}
\vspace{-3mm}
\label{tab:Crossmadal3600}
{
\begin{tabular}{cccc}
\toprule
\textbf{Method}  &\textbf{Data} & \textbf{I2T}  & \textbf{T2I}  \\
\hline
\multicolumn{4}{c}{\textbf{\textit{Model Architecture: CLIP ViT-B/32}}} \\
\hline

LLM2CLIP &3M &  39.9 & 40.3 \\
ProVLA & 3M & 43.8 & 43.0 \\


\multicolumn{4}{c}{\textbf{\textit{Model Architecture: CLIP ViT-B/16}}} \\
\hline

LLM2CLIP &3M &  43.7 & 43.1 \\
ProVLA & 3M & 45.6 & 44.0 \\


\multicolumn{4}{c}{\textbf{\textit{Model Architecture: CLIP ViT-L/14}}} \\
\hline

LLM2CLIP &3M &  46.6 & 44.2 \\
ProVLA & 3M & 49.1 & 46.1 \\


\multicolumn{4}{c}{\textbf{\textit{Model Architecture: EVA02-CLIP ViT-L/14}}} \\
\hline

LLM2CLIP &3M &  48.9   & 47.4 \\
ProVLA & 3M & 50.6 & 47.9 \\


\bottomrule
\end{tabular}
}
\vspace{-3mm}
\end{table*}

==> Table/reg_weight.tex <==
\begin{table}[t!]
    \centering
    \caption{Ablation of $\mathcal{L}_{reg}$}
    \setlength{\tabcolsep}{3pt}
    \resizebox{0.6\linewidth}{!}{
    \begin{tabular}{ccccc}
    
    \toprule
    \textbf{$\lambda_{reg}$} & \textbf{IN-1k} & \textbf{I2T Avg.} & \textbf{T2I Avg.}\\
    \midrule
    0    & 59.2  & 82.9 & 80.2 \\
    \midrule 
    2e-4 & 60.3 & 82.8 & 80.3 \\
    \rowcolor[rgb]{0.925,0.957,1}
    4e-4  & 62.5 & \textbf{83.0} & \textbf{80.5} \\
    6e-4  & \textbf{62.6} & 82.6 & 79.8 \\
    1e-3 &  62.5 & 81.8 & 79.5\\
    \bottomrule
    \end{tabular}
    }
    \vspace{-2mm}

    \label{tab:reg_weight}
\end{table}

==> Table/robustness.tex <==

\begin{table}[t!]
\centering
\caption{Robustness performance. The best results are marked in \textbf{bold}.}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{lccccccc}
\toprule
\multirow{2}{*}{\textbf{Method}}  &\multirow{2}{*}{\textbf{\#Data}} & \multicolumn{5}{c}{\textbf{Robustness}} \\

& &  \textbf{IN-V2} &  \textbf{IN-A} &   \textbf{IN-O}&   \textbf{IN-R}&\textbf{IN-S} \\
\midrule
\multicolumn{4}{l}{\textit{Model Architecture: CLIP ViT-L/14}} & &   \\
\textcolor{gray}{CLIP} & 
\textcolor{gray}{400M} & 
\textcolor{gray}{69.8} & 
\textcolor{gray}{70.8} & 
\textcolor{gray}{32.2} & 
\textcolor{gray}{87.8} & 
\textcolor{gray}{59.6} \\

LLM2CLIP &3M &  49.0 & 46.6 & 32.4 & 75.0 & 44.8 \\
\rowcolor[rgb]{0.925,0.957,1}\modelnm\ & 3M & 
\textbf{58.3} &
\textbf{63.3} & 
\textbf{31.6} & 
\textbf{84.0} & 
\textbf{52.3} \\
\hdashline
LLM2CLIP &15M &  50.8 & 50.1 & 33.8 & 78.2 & 46.3 \\
\rowcolor[rgb]{0.925,0.957,1}\modelnm\ & 15M & 
\textbf{62.1} & 
\textbf{66.4} & 
\textbf{34.2} & 
\textbf{86.4} & 
\textbf{55.3} \\
\hdashline
LLM2CLIP &30M & 52.7 & 52.7 & 34.0 & 78.6 & 47.3 \\
\rowcolor[rgb]{0.925,0.957,1}\modelnm\ & 30M & 
\textbf{63.4} & 
\textbf{68.0} & 
\textbf{34.1} & 
\textbf{86.8} & 
\textbf{55.7} \\

\bottomrule
\end{tabular}
}

\vspace{-5mm}
\label{tab:roubutness}
\end{table}



==> Table/roubutness_new.tex <==
\begin{table*}[t!]
\centering
\caption{Roubutness performance.  The best results are marked in bold}
\vspace{-3mm}
\label{tab:roubutness}
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{lcccccc|c}
\toprule
\textbf{Method}  &\textbf{Data} &  \textbf{IN-v2} &  \textbf{IN-A} &   \textbf{IN-O}&   \textbf{IN-R}&\textbf{IN-S} & \textbf{Avg.} \\
\hline
\multicolumn{8}{c}{\textbf{\textit{Model Architecture: CLIP ViT-B/32}}} \\
\hline
\textcolor{gray}{CLIP} & 
\textcolor{gray}{400M} & 
\textcolor{gray}{55.9} & 
\textcolor{gray}{31.6} & 
\textcolor{gray}{47.8} & 
\textcolor{gray}{69.3} & 
\textcolor{gray}{42.3} & 
\textcolor{gray}{49.4} \\

LLM2CLIP &3M &  37.0 & 18.8 & 38.0 & 54.0 & 30.7 & 35.7 \\
ProVLA & 3M & 
\textbf{43.6} & 
\textbf{25.5} & 
\textbf{40.6} & 
\textbf{62.9} & 
\textbf{35.3} & 
\textbf{41.6(+5.9)} \\


\hline
\multicolumn{8}{c}{\textbf{\textit{Model Architecture: CLIP ViT-B/16}}} \\
\hline
\textcolor{gray}{CLIP} & 
\textcolor{gray}{400M} & 
\textcolor{gray}{61.9} & 
\textcolor{gray}{49.9} & 
\textcolor{gray}{42.3} & 
\textcolor{gray}{77.7} & 
\textcolor{gray}{48.2} & 
\textcolor{gray}{56.0} \\

LLM2CLIP &3M &  42.4 & 30.2 & 35.3 & 61.6 & 35.2 & 40.9 \\
ProVLA & 3M & 
\textbf{50.8} & 
\textbf{41.4} & 
\textbf{38.5} & 
\textbf{71.3} & 
\textbf{41.7} & 
\textbf{48.7(+7.8)} \\



\hline
\multicolumn{8}{c}{\textbf{\textit{Model Architecture: CLIP ViT-L/14}}} \\
\hline
\textcolor{gray}{CLIP} & 
\textcolor{gray}{400M} & 
\textcolor{gray}{69.8} & 
\textcolor{gray}{70.8} & 
\textcolor{gray}{32.2} & 
\textcolor{gray}{87.8} & 
\textcolor{gray}{59.6} & 
\textcolor{gray}{64.0} \\

LLM2CLIP &3M &  49.0 & 46.6 & 32.4 & 75.0 & 44.8 & 49.5 \\
ProVLA & 3M & 
\textbf{58.3} & 
\textbf{63.3} & 
\textbf{31.6} & 
\textbf{84.0} & 
\textbf{52.3} & 
\textbf{57.9(+8.4)} \\





\hline
\multicolumn{8}{c}{\textbf{\textit{Model Architecture: Eva02-CLIP ViT-L/14}}} \\
\hline
\textcolor{gray}{Eva02-CLIP} & 
\textcolor{gray}{2B} & 
\textcolor{gray}{72.6} & 
\textcolor{gray}{76.4} & 
\textcolor{gray}{29.6} & 
\textcolor{gray}{92.7} & 
\textcolor{gray}{67.9} & 
\textcolor{gray}{67.8} \\

LLM2CLIP & 3M & 51.8 & 50.4 & 28.8 & 79.1& 50.6 & 52.1 \\
ProVLA & 3M & 
\textbf{62.0} & 
\textbf{66.5} & 
\textbf{29.3} & 
\textbf{89.4} & 
\textbf{59.9} & 
\textbf{61.4(+9.3)} \\

\bottomrule
\end{tabular}
}
\vspace{-3mm}
\end{table*}

==> Table/sugar_crepe.tex <==
\begin{table*}[t!]
\centering
\caption{SugarCrepe performance.  The best results are marked in bold.}
\vspace{-3mm}
\label{tab:sugar_crepe}
\resizebox{0.6\linewidth}{!}{
\begin{tabular}{lcccc}
\toprule
\textbf{Method}  &\textbf{Data} &\textbf{Add} &\textbf{Replace} &\textbf{Swap} \\  






\hline
\textit{Model Architecture: CLIP ViT-L/14} \\
\textcolor{gray}{CLIP} & 
\textcolor{gray}{400M} & 
\textcolor{gray}{74.8} & 
\textcolor{gray}{79.4} & 
\textcolor{gray}{61.0} \\

LLM2CLIP &3M &  89.9 & 90.0 & 73.7\\
\rowcolor[rgb]{0.925,0.957,1}
ProVLA & 3M & \textbf{92.5\textcolor{kcgreen}{(+2.6)}} & \textbf{90.7\textcolor{kcgreen}{(+0.7)}} & \textbf{75.5\textcolor{kcgreen}{(+1.8)}}\\

\hline
\textit{Model Architecture: Eva02-CLIP ViT-L/14} \\
\textcolor{gray}{CLIP} & 
\textcolor{gray}{400M} & 
\textcolor{gray}{86.6} & 
\textcolor{gray}{70.0} & 
\textcolor{gray}{62.2} \\

LLM2CLIP &3M &   91.3& 89.8 & 74.1\\
\rowcolor[rgb]{0.925,0.957,1}
ProVLA & 3M & \textbf{92.0\textcolor{kcgreen}{(+0.7)}} & \textbf{90.4\textcolor{kcgreen}{(+0.6)}} & \textbf{77.6\textcolor{kcgreen}{(+3.5)}}\\



\bottomrule
\end{tabular}
}
\vspace{-5mm}
\end{table*}

==> Table/table1.tex <==
\begin{table}[t!]
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{cc c cc}
    \toprule
    Text Encoder & Vision Encoder & Data & Classification (Avg 11) & Retrieval (Avg 8) \\
    \midrule
        Openai CLIP-L-14 & Openai CLIP-L-14 & WiT400M &  75.9 & 49.9 \\
        Nvembedv2 7B & DINOv2-L & 23M(cc3M+12M,Yfcc15M) & 72.7 & 63.9\\
        Openai CLIP-B-16 & Openai CLIP-B-16& WiT400M &  63.7 & 43.5 \\
        Mistral 7B & Openai CLIP-B-16 & 3M(cc3m) & 39.5 & 42.3\\
        Llama cc 8B & Openai CLIP-L-14 & 60M(cc3M+12M,Yfcc15M,LAION-30M) &  69.9 & 69.5 \\
        \midrule
        Llama cc 8B & Openai CLIP-L-14 & 15M(cc3M+cc12M) &  57.5 & 67.8 \\
        Nvembedv2 7B & Openai CLIP-L-14 & 15M(cc3M+cc12M) &  56.2 & 67.0 \\
        Nvembedv2 7B & DINOv2-L & 15M(cc3M+cc12M) &  48.4 & 62.2 \\        
        Gme(MLLM-based) 7B & Openai CLIP-L-14 & 15M(cc3M+cc12M) &  56.8 & 66.8 \\
        Qwen-Embedding 0.6B & Openai CLIP-L-14 & 15M(cc3M+cc12M) &  43.1 & 62.2 \\
        Qwen-Embedding 4B & Openai CLIP-L-14 & 15M(cc3M+cc12M) &  51.1 & 64.7 \\
        Qwen-Embedding 8B & Openai CLIP-L-14 & 15M(cc3M+cc12M) &  53.7 & 65.9 \\ 
    \bottomrule
    \end{tabular}
    }
    \caption{Combination of different encoders}
    \label{tab:encoder}
\end{table}


==> Table/table1_new.tex <==
\begin{table*}[ht]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{l c | cc | cc | cc | cc | cc | ccc}
\shline
\multirow{2}{*}{\textbf{Methods}} & \multirow{2}{*}{\textbf{LLM}} & \multicolumn{2}{c|}{\textbf{Flickr30k}} & \multicolumn{2}{c|}{\textbf{COCO}} & \multicolumn{2}{c|}{\textbf{ShareGPT4V}} & \multicolumn{2}{c|}{\textbf{Urban-1k}} & \multicolumn{2}{c|}{\textbf{DOCCI}} & \multicolumn{2}{c}{\textbf{Average}} & \multirow{2}{*}{\textbf{Class Avg.}}\\
 &  & \textbf{I2T} & \textbf{T2I} & \textbf{I2T} & \textbf{T2I} & \textbf{I2T} & \textbf{T2I} & \textbf{I2T} & \textbf{T2I} & \textbf{I2T} & \textbf{T2I} & \textbf{I2T} & \textbf{T2I} \\
\shline
\multicolumn{14}{l}{\textbf{ViT-B/16(86M)}} \\
\hline
CLIP~\cite{radford2021learning}                      & - & 79.9 & 60.0 & 51.7 & 30.2 & 69.7 & 62.4 & 62.3 & 46.5 & 49.7 & 53.2 & 58.0 & 55.1  & 63.7\\

\rowcolor[rgb]{0.925,0.957,1}\hspace{3mm}+FLAME-3M 
                          & mistral 7B & 66.5 & 52.1 & 35.4 & 24.1 & 74.7 & 80.5 & 61.2 & 60.3 & 41.0 & 40.5 & 55.8 & 51.5 & 39.5 \\                          
\hline
\multicolumn{14}{l}{\textbf{ViT-L/14 (307M)}} \\
\hline

CLIP~\cite{radford2021learning}                       & - & 86.6 & 64.6 & 57.2 & 36.4 & 68.7 & 78.0 & 56.0& 68.4 & 63.1 & 65.8 & 66.3 & 62.6  & 75.7\\
\rowcolor[rgb]{0.925,0.957,1}\hspace{3mm}+\ourmethod{}-15M 
                          & Llamacc 8B & 91.2 & 80.8 & 67.5 & 51.7 & 95.7 & 96.0 & 91.7 & 87.2 & 89.0 & 87.2 & 87.0 & 80.6 & 57.5\\
\rowcolor[rgb]{0.925,0.957,1}\hspace{3mm}+\ourmethod{}-15M 
                          & Nvembedv2 7B& 91.2 & 80.6 & 64.8 & 51.1 & 94.8 & 95.3 & 90.9 & 89.1 & 85.3 & 84.3 & 85.4 & 80.1 & 56.2\\
\rowcolor[rgb]{0.925,0.957,1}\hspace{3mm}+\ourmethod{}-15M 
                          & Gme (MLLM-based) 7B& 91.3 & 78.8 & 66.5 & 50.1 & 95.7 & 95.5 & 92.4 & 91.4 & 86.4 & 85.4 & 86.5 & 80.3 & 56.8\\

                          
\rowcolor[rgb]{0.925,0.957,1}\hspace{3mm}+\ourmethod{}-15M 
                          & Qwen 0.6B & 77.7 & 65.9 & 46.4 & 31.4  & 88.8 & 88.4 & 67.2 & 62.2 & 51.8 & 49.1 & 66.4 & 59.4& 43.1\\
\rowcolor[rgb]{0.925,0.957,1}\hspace{3mm}+\ourmethod{}-15M 
                          & Qwen 4B & 88.9 & 78.0 & 62.2 & 48.6 & 95.0 & 95.4 & 88.7 & 84.6 & 82.7 & 79.9 & 83.5& 77.3 & 51.1\\
\rowcolor[rgb]{0.925,0.957,1}\hspace{3mm}+\ourmethod{}-15M 
                          & Qwen 8B & 91.4 & 79.4 & 63.5 & 49.8 & 95.2 & 96.0 & 90.3 & 89.6 & 85.0 & 82.4 & 85.1 & 79.4 & 53.7\\                          

                          

                        

                          
\rowcolor[rgb]{0.925,0.957,1}\hspace{3mm}+Image distill 
                          & Llamacc 8B & 89.8 & 80.7 & 64.7 & 49.6 & 94.9 & 95.8 & 90.0 & 85.2 & 86.3 & 84.9 & 85.1 & 79.3  & 60.1\\
\rowcolor[rgb]{0.925,0.957,1}\hspace{3mm}+Text distill
                          & Llamacc 8B & 92.1 & 81.8 & 69.0 & 52.2 & 93.3 & 94.5 & 91.5 & 86.9 & 88.2 & 87.6 & 86.8 & 80.6 & 60.5 \\
\rowcolor[rgb]{0.925,0.957,1}\hspace{3mm}+Image Distill+ Text distill
                          & Llamacc 8B & 91.4 & 81.0 & 66.6 & 51.2 & 95.5 & 95.7 & 91.6 & 86.4 & 87.4 & 86.1 & 86.5 & 80.1 & 63.6 \\
\rowcolor[rgb]{0.925,0.957,1}\hspace{3mm}+Image Distill+ Text distill + 0.2 Noise text
                          & Llamacc 8B & 92.1 & 81.0 & 67.2 & 52.0 & 94.9 & 95.0 & 91.7 & 87.6 & 87.8 & 85.5 & 86.7 & 80.2 & 66.8 \\
DINOv2~\cite{dinov2}+sail-23M & Nvembdv2 7B & 87.8 & 74.5 & 62.7 & 46.6 & 90.1 & 92.3 & 82.8& 83.7 & 78.6 & 76.1 & 80.4 & 74.6 & 72.7\\
\rowcolor[rgb]{0.925,0.957,1}\hspace{3mm}+\ourmethod{}-15M 
                          & Nvembedv2 7B & 88.8 & 76.6 & 59.7 & 47.4 & 93.5 & 93.3 & 84.9 & 80.1 & 79.6 & 76.2 & 81.3 & 74.7 & 48.4 \\
\shline
\end{tabular}%
}
\caption{Systematic comparison of model performance on multiple datasets. The light blue row indicate~\ourmethod{} post trained version. }
\label{tab:sys_compare}
\end{table*}

==> Table/table2.tex <==
\begin{table}[t!]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{cccccc}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{ } & \multicolumn{2}{c}{Llama cc 8B} & \multicolumn{2}{c}{Nvembedv2 7B} \\
\cline{3-6}
 &  & Classification (Avg 11) & Retrieval (Avg 8) & Classification (Avg 11) & Retrieval (Avg 8) \\
\midrule
Direct Finetune & & 57.5 & 67.8 & 56.2 & 67.0\\
Lock Image Tuning & & - & - & 60.0 & 62.7 \\
+Image distill & & 60.1 & 66.5 & 58.6 & 66.6 \\
\midrule
+Text distill mse & & 60.5 & 67.6 & 59.2 & 68.5 \\
+Text distill cos & & - & - & 59.3 & 66.8 \\
+Text distill with long & & - & - & 58.2 & 66.9 \\
\midrule
+Image distill + Text distill & & 63.6 & 66.9 & 62.4 & 67.2 \\
+Image distill + Text distill + Add noise text & & 66.8 & 67.3 & 65.9 & 67.3 \\
\bottomrule
\end{tabular}
}
\caption{Comparison between Llama cc 8B and Nvembedv2 7B under different distillation methods.}
\label{tab:comparison}
\end{table}


==> Table/table2_new.tex <==
\begin{table*}[ht]
\centering
\renewcommand{\arraystretch}{1.2} %
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|cc|cc|cc|cc|cc|cc}
\shline
\multirow{2}{*}{\textbf{Methods}} & \multicolumn{2}{c|}{\textbf{Flickr}} & \multicolumn{2}{c|}{\textbf{COCO}} & \multicolumn{2}{c|}{\textbf{ShareGPT4V}} & \multicolumn{2}{c|}{\textbf{Urban-1k}} & \multicolumn{2}{c|}{\textbf{DOCCI}} & \multicolumn{2}{c}{\textbf{Average}} \\
                                  & \textbf{I2T} & \textbf{T2I} & \textbf{I2T} & \textbf{T2I} & \textbf{I2T} & \textbf{T2I} & \textbf{I2T} & \textbf{T2I} & \textbf{I2T} & \textbf{T2I} & \textbf{I2T} & \textbf{T2I} \\
\shline
CLIP                               & 89.6 & 77.8 & 59.4 & 48.6 & 88.1 & 87.7 & 68.0 & 74.8 & 67.0 & 71.3 & 74.4 & 72.0 \\
Directly Finetune(50\%)             & 89.3 & 77.8 & 59.3 & 48.5 & 88.3 & 88.2 & 68.5 & 76.0 & 67.2 & 71.2 & 74.5 & 72.3 \\
\hline
bge-en-icl                         & 89.1 & 78.5 & 58.8 & 49.7 & 95.0 & 95.7 & 77.9 & 87.7 & 73.5 & 79.4 & 78.9 & 78.2 \\
LLM2Vec-Llama-3-8B & 91.1 & 81.4 & 61.5 & 51.9 & 94.5 & \textbf{96.4} & 82.1 & 88.6 & 77.7 & 82.6 & 81.4 & 80.2 \\
NV-Embed-v2                        & 90.4 & 80.0 & 60.5 & 51.6 & 94.5 & 95.7 & 83.3 & \textbf{90.0} & 78.3 & 82.1 & 81.4 & 79.9 \\
\hline
Qwen2.5-0.5B-CC                    & 86.2 & 74.9 & 56.0 & 45.1 & 92.6 & 93.2 & 73.7 & 79.0 & 69.5 & 73.0 & 75.6 & 73.0 \\
Llama-3.2-1B-CC                    & 88.9 & 78.8 & 59.8 & 49.1 & 96.3 & 95.6 & 80.1 & 85.1 & 77.0 & 80.8 & 80.4 & 77.9 \\
Llama-3-8B-CC                      & 90.4 & 80.7 & 62.7 & 51.9 & 96.5 & 96.2 & 84.2 & 89.5 & 83.3 & \textbf{86.4} & 83.4 & 80.9 \\
DeepSeek-R1-Distill-Llama-8B-CC     & 91.7 & 80.9 & 62.2 & 51.9 & 96.7 & 96.3 & 84.3 & 88.3 & 82.5 & 85.2 & 83.5 & 80.5 \\
Llama-3.1-8B-CC                    & \textbf{92.2} & \textbf{81.5} & \textbf{63.5} & \textbf{52.3} & \textbf{97.1} & 96.2 & \textbf{86.5} & 89.3 & \textbf{84.7} & 85.9 & \textbf{84.8} & \textbf{81.0} \\
\rowcolor{red!20} \textcolor{red}{Llama3.1-8B}                    & 85.2 & 74.6 & 52.3 & 40.8 & 87.7 & 89.6 & 57.5 & 59.2 & 49.9 & 48.3 & 66.5 & 62.5 \\
\shline
\end{tabular}%
}
\caption{Ablation for using different text encoder. BGE-EN-ICL, LLM2Vec-Llama-3-8B, and NV-Embed-v2 are community-released text encoders derived from LLMs. The suffix "-CC" indicates encoders that have undergone our caption contrastive fine-tuning method based on the respective original LLMs. }
\label{tab:llm_encoders}
\end{table*}
